A* search algorithm for an optimal investment problem in vehicle-sharing systems

We study an optimal investment problem that arises in the context of the vehicle-sharing system. Given a set of locations to build stations, we need to determine i) the sequence of stations to be built and the number of vehicles to acquire in order to obtain the target state where all stations are built, and ii) the number of vehicles to acquire and their allocation in order to maximize the total profit returned by operating the system when some or all stations are open. The profitability associated with operating open stations, measured over a specific time period, is represented as a linear optimization problem applied to a collection of open stations. With operating capital, the owner of the system can open new stations. This property introduces a set-dependent aspect to the duration required for opening a new station, and the optimal investment problem can be viewed as a variant of the Traveling Salesman Problem (TSP) with set-dependent cost. We propose an A* search algorithm to address this particular variant of the TSP. Computational experiments highlight the benefits of the proposed algorithm in comparison to the widely recognized Dijkstra algorithm and propose future research to explore new possibilities and applications for both exact and approximate A* algorithms.

==> irgnore-model-properties.tex <==
\subsection{Semi-Markov Decision Process for Determining the Optimal Fleet Size}
We see the optimal investment scheduling problem of AMoD operators as a Semi-Markov Decision Process (SMDP) because of the nature of the investment problem. In an SMDP, the system's state evolves over time according to a semi-Markov process, and the decision-maker selects actions based on the current state. Let $\mathcal{S}$ be the set of states of the process. Each state $s\in\mathcal{S}$ describes the current fleet size $n$ and the currently opened stations, given by $x_i = 1$ if station $i\in\mathcal{I}$ is open, $0$ otherwise; or $s = \langle n, x_1, \dots, x_I\rangle$. 

Each state $s$ is associated with an operational profit $\pi_s$ per time period, which is calculated by subtracting the rebalancing costs from the contribution margins. 
% The computation method for $\pi_s$ is not provided here but will be explained later in the paper. 
Only states with a positive operational profit ($\pi_s > 0$) are considered for the optimal investment schedule, except for the starting state $s_0$, which has an operational profit of $\pi_{s_0} = 0$. The set of states with positive operational profit and the starting state is denoted as $\mathcal{S}$. For referencing the fleet size and open stations of a specific state $s$, the notation $n\left(s\right)$ and $x_i\left(s\right)$ are utilized, respectively.
\subsubsection*{Actions}
Actions refer to the operator's procurement decision, resulting in a state transition into the target state $t\in\mathcal{S}$. Every state $s\in\mathcal{S}\setminus\{s_0\}$ permits transitions to all other states such that no stations are being closed, i.e., $s\rightarrow t$ exists iff $x_i\left(s\right) \leq x_i\left(t\right) \forall i$, and there is precisely one action that results in every state transition. From state $s_0$, the system can transmit to every state such that the investment volume does not exceed the budget $B$. 
% Thus, for simplicity, we omit actions from the necessary notation and henceforth use origin state $s$ and target state $t$ whenever we refer to an action. 
The time $\tau_{st}$ necessary for a state transition depends on the operational profit $\pi_s$ and the necessary investment volume $C_{st}$ where 
\begin{align*}
C_{st} = \left(n\left(t\right) - n\left(s\right)\right)\cdot c^p + \sum_{i \in I}\left(1 - x_i\left(s\right)\right) \cdot x_i\left(t\right)\cdot c^b
\end{align*}
Given that we do not consider partial states (e.g., a state without optimal fleet size), the optimal decision is always to transition to the next state as soon as possible. Thus, 
\begin{align*}
\tau_{st} = \frac{C_{st}}{\pi_s}
\end{align*}

% Actions correspond to the procurement decisions made by the operator, leading to a transition from the current state to the next state $t\in\mathcal{S}$. For every state $s\in\mathcal{S}\setminus{s_0}$, transitions to other states are possible as long as no stations are being closed. In other words, a transition $s\rightarrow t$ exists if and only if $x_i\left(s\right) \leq x_i\left(t\right)$ for all stations $i$, and there is precisely one action associated with each state transition. When starting from state $s_0$, the system can transition to any state if the investment cost does not exceed the budget $B$.

% To simplify the notation, actions are omitted, and the origin state $s$ and target state $t$ are used to refer to an action. The time $\tau_{st}$ required for a state transition depends on the operational profit $\pi_s$ and the investment cost $C_{st}$, where:
% \begin{align*}
% C_{st} = \left(n\left(t\right) - n\left(s\right)\right)\cdot c^p + \sum_{i \in I}\left(1 - x_i\left(s\right)\right) \cdot x_i\left(t\right)\cdot c^b.
% \end{align*}
% % Clearly, the optimal decision is always to transition to the next state as soon as possible. Thus, 
% % \begin{align*}
% % \tau_{st} = \frac{C_{st}}{\pi_s}.
% % \end{align*}

% Clearly, the optimal decision is always to transition to the next state as soon as possible. Thus, 
% \begin{align*}
% \tau_{st} = \frac{C_{st}}{\pi_s}.
% \end{align*}


\subsection{Mathematical model for calculating optimal profit and minimum acquisition cost}
To compute the operational profit $\pi_s$ for $s\in\mathcal{S}$, we formulate our problem as an optimization problem over an open queueing network. It shares similarities with formulations mentioned in \cite{braverman2019empty,hao2021prohibiting,he2017service}. Given open stations, we give the model full control over the fleet size and the distribution of vehicles. Since we want to maximize profit and minimize the corresponding acquisition cost, our objective function will be hierarchical.  
% \ref{hao2021prohibiting} where we consider an open queueing network (receive customers from an external source and send them to an external destination) instead of a closed queueing network \cite{braverman2019empty} (a fixed population that moves between the queues but never leaves the system) to present the nature of the bike-sharing systems. \cite{hao2021prohibiting,he2017service}, we assume that open stations are given. We ensure the minimum level of service, $\alpha$, in our model while in \cite{hao2021prohibiting} XXX, 
% In this open queueing network, vehicles correspond to ``customers'' and servers correspond to ``stations''. 
% The AMoD system's customers are modeled as arrival rates at the stations $i$, transferring to another station $j$. 
To determine the maximal operational profit per period of time for state $s$, we solve \eqref{eq:objectiveRebalancing}-\eqref{eq:domain1} for all open stations $\mathcal{I}^{\vec{x}} = \{i | x_i\left(s\right) = 1\}$ where $\vec{x} = \langle x_1\left(s\right),\dots x_I\left(s\right)\rangle$. 
We denote $f_{ij}, e_{ij}$ as the number of occupied and empty vehicles traveling from $i$ to $j$. Together with other factors (costs, traveling rates), those values help determine the profit we want to calculate.
% \cite{braverman2019empty,hao2021prohibiting} we use the decision variables $e_{ij},i\neq j$ for the number of empty vehicles rebalancing from $i$ to $j$ (and hence, $e_{ii}$ for the number of empty vehicles currently parked at the station (or region) $i$). Similarly, we 

% \minhvd{$f_{ii} = 0$ It is correct or not?}

% A upper bound for rebalancing costs: 
% \begin{align}
% E = \sum_{i,j\in I}{\left(x_i x_j \max{\left(\lambda_{ij} - \lambda_{ji},0\right)} \max_{k\in I}{c_{ik}}\right)}
% \end{align}


\begin{multline}
    P(obj_1,obj_2) = \Bigl(\max \,\,\, \alpha \Bigl( \sum_{i\in\mathcal{I}^{\vec{x}}} \sum_{j\in\mathcal{I}^{\vec{x}}}{\lambda_{ij}\left(\vec{x}\right)r_{ij}} \\ -\sum_{i\in\mathcal{I}^{\vec{x}}}\sum_{j\in\mathcal{I}^{\vec{x}}}{c_{ij}\mu_{ij}e_{ij}} \Bigl),\min \,\,\,  \Bigl( n*c_p+\sum_{i\in\mathcal{I}^{\vec{x}}}c_b^i \Bigl) \Bigl)
    \label{eq:objectiveRebalancing}
\end{multline}
subject to
\begin{align}
\lambda_{ij} \left(\vec{x}\right)&=\mu_{ij}f_{ij} &\forall i,j\in\mathcal{I}^{\vec{x}}\label{eq:fullCarLittlesLaw} \\
%empty car i-j Little's Law relaxation
\sum_{k\in\mathcal{I}^{\vec{x}\setminus\{i\}}}\mu_{ki}e_{ki} &\leq \sum_{j\in\mathcal{I}^{\vec{x}}}\lambda_{ij}\left(\vec{x}\setminus\{i\}\right) &\forall i\in\mathcal{I}^{\vec{x}}\label{eq:emptyCarLittlesLaw} \\
\sum_{j\in\mathcal{I}^{\vec{x}}}\lambda_{ij}\left(\vec{x}\right)+\sum_{j\in\mathcal{I}^{\vec{x}}}\mu_{ij}e_{ij}&=   \sum_{k\in\mathcal{I}^{\vec{x}}}^r\mu_{ki}e_{ki} + \sum_{k\in\mathcal{I}^{\vec{x}}}\mu_{ki}f_{ki}\,\,\, &\forall i\in\mathcal{I}^{\vec{x}}\label{eq:carFlowBalance2}\\ 
\frac{\alpha}{1-\alpha} &\leq e_{ii} &\forall i\in\mathcal{I}^{\vec{x}}\label{eq:actualavailability2} \\
%fleet dimension control
\sum_{i,j\in\mathcal{I}^{\vec{x}}}{\left(e_{ij}+f_{ij}\right)}&=n\label{eq:fleetDimension} \\
%unit definition
e_{ij}, f_{ij}  &\geq 0 &\forall i,j\in\mathcal{I}^{\vec{x}}\label{eq:domain1}
\end{align}
 
The objective function \eqref{eq:objectiveRebalancing} maximizes the profit which consists of the contribution margin of all served customers minus rebalancing costs, multiplied by the availability $\alpha$ to account for those customers who cannot be served; and then minimize the corresponding set up cost. Constraints \eqref{eq:fullCarLittlesLaw}-\eqref{eq:carFlowBalance2} are linearizations of the flow constraints in queueing networks and almost directly follow from \cite{braverman2019empty}. Unlike \cite{braverman2019empty}, we require that the system must achieve a service level of at least $\alpha$, and thus remove any notion of an upper bound on demand. Constraints \eqref{eq:actualavailability2} set the required ``safety stock'', i.e. the number of vehicles that must remain at station $i$ in the steady state to fulfill at least a fraction $\alpha$ of the demand. These constraints follow from the fixed population mean approximation in open queueing networks, and are due to \cite{whitt1984open}. Constraint \eqref{eq:fleetDimension} bounds the fleet size, and constraints \eqref{eq:domain1} define the domain. 

% From \eqref{eq:fullRebalancingModel}, it becomes clear that for each set of open stations, there is exactly one optimal fleet size. This fleet size corresponds to the minimal real-valued $n$ such that \eqref{eq:fullRebalancingModel} has a solution. However, for simplicity and readability we keep $n$ in the state description. 

% To compute the target state $t$, i.e. the optimal state if there were no capital restrictions and the state that the AMoD system will eventually reach over time, follows from \eqref{eq:fullRebalancingModel} if the open regions and the fleet size become strategic as well, analogous to \cite{hao2021prohibiting,he2017service} where the former additionally permit a strategic choice of service level. 
% \eqref{eq:fullRebalancingModel} for all open stations $\mathcal{I}^{\vec{x}} = \{i | x_i\left(s\right) = 1\}$ where $\vec{x} = \langle x_1\left(s\right),\dots x_I\left(s\right)\rangle$. 
% \begin{subequations}\label{eq:fullRebalancingModel}
% \begin{align}
% % \max&\quad \alpha\left(\sum_{i\in\mathcal{I} } \sum_{j\in\mathcal{I} }{\lambda_{ij}r_{ij}}-\sum_{i\in\mathcal{I} }\sum_{j\in\mathcal{I}\setminus\{i\}}{c_{ij}\mu_{ij}e_{ij}}\right)\label{eq:objectiveRebalancing} 
% \max&\quad \sum_i  b_i \label{eq:objectiveRebalancing} 
% \\
% \intertext{subject to}
% %full car i-j Little's Law
% \lambda_{ij}b_{ij} &=\mu_{ij}f_{ij} &\forall i,j\in\mathcal{I} \label{eq:fullCarLittlesLaw} \\
% %empty car i-j Little's Law relaxation
% \sum_{k\in\mathcal{I} \setminus\{i\}}\mu_{ki}e_{ki} &\leq \sum_{j\in\mathcal{I} }\lambda_{ij}b_{ij} &\forall i,j\in\mathcal{I} \label{eq:emptyCarLittlesLaw} \\
% %car flow balance region i relaxation
% %\sum_{j\in\mathcal{I}}\lambda_{ij} &\leq \sum_{k\in\mathcal{I}\setminus\{i\}}\mu_{ki}e_{ki} + \sum_{k\in\mathcal{I}}\mu_{ki}f_{ki} &\forall i\in\mathcal{I}\label{eq:carFlowBalance1} \\
% \sum_{j\in\mathcal{I} }\lambda_{ij}b_{ij}+\sum_{j\in\mathcal{I}^{\vec{x}}\setminus\{i\}}\mu_{ij}e_{ij}&=\sum_{k\in\mathcal{I} \setminus\{i\}}^r\mu_{ki}e_{ki} + \sum_{k\in\mathcal{I} \setminus\{i\}}\mu_{ki}f_{ki} &\forall i\in\mathcal{I} \label{eq:carFlowBalance2} \\
% %link availability and fleet size (FPM)
% \frac{\alpha}{1-\alpha}b_i &\leq e_{ii} &\forall i\in\mathcal{I} \label{eq:actualavailability2} \\
% %fleet dimension control
% \sum_{i,j\in\mathcal{I}^{\vec{x}}}{\left(e_{ij}+f_{ij}\right)}&=n\label{eq:fleetDimension} \\
% %unit definition
% e_{ij} \leq M*b_{ij}, \forall i \in I \\
% f_{ij} \leq M*b_{ij}, \forall i \in I \\
% \sum_{i} b_i*c_i^b + n*c^p \leq B \\
% e_{ij}, f_{ij}  &\geq 0 &\forall i,j\in\mathcal{I}\\
% \label{eq:domain1} 
% \end{align}
% \end{subequations}

  
\subsection{Solution Algorithm based on Shortest Paths}
% The AMoD operator aims at maximizing \textcolor{red}{her} profit. There exists an optimal state $s^\prime\in\mathcal{S}$ with maximal operational profit per period of time. Once the AMoD system reaches this optimal fleet size and optimal set of open stations, the operator will no longer change the system state. 
% Formally, the operator's problem is thus equivalent to traversing the state space with the goal of reaching the target state $t$ as fast as possible. A solution to our problem looks like a solution to the classic Traveling Salesman Problem, which can be seen as a permutation of $n$ stations. Some first stations can be acquired using the budget $B$, while the remaining stations will be acquired one by one when having additional capital. The problem is then like a TSP with order-dependent cost (or set-dependent cost since transition time from a state $s$ to a state $t$ depending on the set of opening stations in $s$.  Therefore, unless using an exponential number of variables, it seems not be easy to model the problem as a mixed integer problem because of the set-dependent cost. So state-of-art solvers such as Gurobi, Cplex limit its application . Therefore, we develop other solutions approaches by considering the current problem as a shortest path problem in a state graph where each state correspond to a sequence of stations $(u_1,u_2,..,u_k)$ in which $u_i$ will be open not later than  $u_j$ if $i<j$.   Unlike road networks with only few connecting edges, the number of actions in each state is large. Also, the triangular inequality does not hold. 
% To solve the problem, we develop and experiment several strategies including heuristics and A* to solve the problem. 
% Therefore, most existing algorithms for shortest path problems are not applicable in this case.

% Thus, we implement Dijkstra's algorithm \citep{dijkstra1959note}, and focus on reducing the size of the graph. 

% In the following, we give three properties of optimal state transitions and states that are part of the shortest path. All states and state transitions which do not possess these properties can therefore be omitted. 
% % (i) In an optimal investment schedule, the operator will never enter a state with a lower operational profit. (ii) In an optimal investment schedule, the operator adds additional stations as quickly as possible. (iii) In an optimal investment schedule, the operator opens as many stations as possible with the budget $B$. 

% \begin{lemma}\label{lemma:profitIncrease}
% Only those state transitions $s\rightarrow t$ such that $\pi_s \leq \pi_t$ are part of the optimal investment schedule. 
% \end{lemma}

% % Please note that state transitions $s\rightarrow t$ with $\pi_s = \pi_t$ do not accelerate the investment schedule, and could therefore also be omitted. However, including these state transitions reduces the number of necessary arcs in the reduced SMDP after applying Lemma \ref{lemma:optimalStateTransitions}.

% \begin{lemma}\label{lemma:optimalStateTransitions}
% Let $s_1$ and $s_m$ be two states such that $x_i\left(s_1\right) = 0, x_i\left(s_m\right) = 1\forall i\in \mathcal{I}^\prime\subset\mathcal{I}$ and $x_i\left(s_1\right) = x_i\left(s_m\right) \forall i\notin \mathcal{I}^\prime\subset\mathcal{I}$ with $|\mathcal{I}^\prime|>1$. 
% Then, the state transition $s_1\rightarrow s_m$ is not optimal unless there exists a path $s_1\rightarrow s_2 \dots \rightarrow s_{m-1}\rightarrow s_m$ such that 
% \begin{itemize}
% \item all transitions $s_{\ell-1}\rightarrow s_\ell, \, \forall \ell = 1,\dots, m-1$ are permitted, 
% \item $\sum_{i\in \mathcal{I}}{|x_i\left(s_\ell\right) - x_i\left(s_{\ell+1}\right)|} = 1,\,\forall \ell = 1,\dots, m-1$, and
% \item $\pi\left(s_{\ell - 1}\right) \leq \pi\left(s_{\ell}\right),\,\forall \ell = 1,\dots, m-1$.
% \end{itemize}
% \end{lemma}

% \begin{lemma}\label{lemma:optimalStartingStates}
% Let $S^\text{B}$ be the set of states that are reachable within the budget limit. If all feasible successors $s_m$ of state $s_1\in S^\text{B}$ are also reachable within the budget limit ($s_m\in S^\text{B}$), state $s_1$ is not part of the optimal path. 
% \end{lemma}

